Modeling Preconditions in Text with a Crowd-sourced Dataset

Preconditions provide a form of logical connection between events that explains why some events occur together and information that is complementary to the more widely studied relations such as causation, temporal ordering, entailment, and discourse relations. Modeling preconditions in text has been hampered in part due to the lack of large scale labeled data grounded in text. This paper introduces PeKo, a crowd-sourced annotation of preconditions between event pairs in newswire, an order of magnitude larger than prior text annotations. To complement this new corpus, we also introduce two challenge tasks aimed at modeling preconditions: (i) Precondition Identification -- a standard classification task defined over pairs of event mentions, and (ii) Precondition Generation -- a generative task aimed at testing a more general ability to reason about a given event. Evaluation on both tasks shows that modeling preconditions is challenging even for today's large language models (LM). This suggests that precondition knowledge is not easily accessible in LM-derived representations alone. Our generation results show that fine-tuning an LM on PeKo yields better conditional relations than when trained on raw text or temporally-ordered corpora.

==> scratch.tex <==

%%%%





\eat{
\begin{table*}[ht!]
    \centering
    \begin{tabular}{c|l|l}
        Error Type & Event Tuple & Sentence \\ \hline \hline
        & \multirow{2}{*}{(the cast, finally \textbf{came}$_{pre}$ off, )}  & When the cast finally \textbf{came}$_{pre}$ off ,  \\
        Extraction & & the patient 's limb would be stiff ... \\
        error  & \multirow{2}{*}{\quad (, to \textbf{get}$_{tgt}$, strength and motion back) }& '' It would take six months of therapy  \\
        & & to \textbf{get}$_{tgt}$ strength and motion back ... \\ \hline
        & \multirow{2}{*}{(few, would \textbf{pick}$_{pre}$, Irma Lara)} & ... few would \textbf{pick}$_{pre}$ Irma Lara . \\
        & & She \textbf{came}$_{tgt}$ to this country \textit{\underline{illegally}} \\
        & \multirow{2}{*}{\quad (She, \textbf{came}$_{tgt}$, to this country)} & \textit{\underline{from a small town in Mexico}}\\
        Missing & & to work as a baby sitter . \\ \cline{2-3}
        context & \multirow{2}{*}{(tax code, will not \textbf{permit}$_{pre}$, a loophole)} &	If the tax code will not \textbf{permit}$_{pre}$\\
        & &  such a loophole , perhaps \textit{\underline{we could}}  \\
        & \multirow{2}{*}{\quad  (you, would \textbf{earn}$_{tgt}$, rewards points)}& \textit{\underline{adopt another popular method}} : ...\\
        & & you would \textbf{earn}$_{tgt}$ rewards points ...\\\hline
        & \multirow{2}{*}{(I, would \textbf{stop}$_{tgt}$, running)} & My husband asked me whether  \\
        & & I would \textbf{stop}$_{tgt}$ running \\
        & \multirow{2}{*}{\quad (the doctor, \textbf{told}$_{pre}$, me to)} & \textit{\underline{if}} the doctor \textbf{told}$_{pre}$ me to . \\
        Missing & & \\ \cline{2-3}
        discourse cue & \multirow{2}{*}{(the guy, would \textbf{face}$_{tgt}$, a few problems)}  & ... the guy born in the church parsonage  \\
        & & that now sits across the street  \\
        & \multirow{2}{*}{\quad (he, were \textbf{running}$_{pre}$, for president)} & from ... would \textbf{face}$_{tgt}$ a few problems \\
        & & \textit{\underline{if}} he were \textbf{running}$_{pre}$ for president .\\\hline
    \end{tabular}
    \caption{Comparison between sentence and tuple models.}
    \label{tab:identification-examples}
\end{table*}
}
\eat{
\begin{table*}[ht!]
    \centering
    \begin{tabular}{c|l}
        Error Type & Input\\ \hline\hline
        & - sentence input \\
         & When the cast finally \textbf{came}$_{pre}$ off ,the patient ’s limb would be stiff ...\\
        Extraction & '' It would take six months of therapy to \textbf{get}$_{tgt}$ strength and motion back ...\\
        error & - tuple input \\
        & (the cast, finally \textbf{came}$_{pre}$ off, ) (, to \textbf{get}$_{tgt}$, strength and motion back) \\ \hline
        & - sentence input \\
        & ... few would \textbf{pick}$_{pre}$ Irma Lara .She \textbf{came}$_{tgt}$ to this country \textit{\underline{illegally from}}\\
        & \textit{\underline{a small town in Mexico}} to work as a baby sitter.\\
        & - tuple input \\
        Missing & (few, would \textbf{pick}$_{pre}$, Irma Lara) (She, \textbf{came}$_{tgt}$, to this country) \\ \cline{2-2}
        context & - sentence input \\
        & If the tax code will not \textbf{permit}$_{pre}$ such a loophole, perhaps \textit{\underline{we could adopt}} \\
        & \textit{\underline{another popular method}} : ...you would \textbf{earn}$_{tgt}$ rewards points ... \\
        & - tuple input \\
        & (tax code, will not \textbf{permit}$_{pre}$, a loophole) (you, would \textbf{earn}$_{tgt}$, reward points) \\ \hline
        & - sentence input \\
        & My husband asked me whether I would \textbf{stop}$_{tgt}$ running \textit{\underline{if}} the doctor \textbf{told}$_{pre}$\\
        & me to. \\
        & - tuple input \\
        Missing & (I, would \textbf{stop}$_{tgt}$, running) (the doctor, \textbf{told}$_{pre}$, me to) \\\cline{2-2}
        discourse cue & - sentence input: \\
        &... the guy born in the church parsonage that now sits across the street\\
        & from ... would \textbf{face}$_{tgt}$ a few problems \textit{\underline{if}} he were \textbf{running}$_{pre}$ for president.\\ 
        & - tuple input: \\
        & (the guy, would \textbf{face}$_{pre}$, a few problem) (he, were \textbf{running}$_{tgt}$, for president) \\ \hline
    \end{tabular}
    \caption{Comparison between sentence and tuple models.}
    \label{tab:identification-examples}
\end{table*}
}

% \begin{table*}[ht!]
%     \centering
%     \begin{tabular}{c|l|l}
%         Error Type & Event Trigger & Event Tuple\\ \hline \hline
%         \multirow{4}{*}{Missing} & \multirow{2}{*}{knew$_{pre}$ missed$_{tgt}$} & (all, \textbf{knew}$_{pre}$, him) \\
%         & & \quad (He, will be deeply \textbf{missed}$_{tgt}$, ) \\
%         context & \multirow{2}{*}{remains$_{pre}$ sign$_{tgt}$}  & (Drew, \textbf{remains}$_{pre}$, a free agent) \\ 
%         & & \quad (he, could \textbf{sign}$_{tgt}$, with another team) \\ \hline
%         & Event Tuple & Sentence \\ \hline \hline
%         \multirow{8}{*}{Extraction} & \multirow{2}{*}{(the cast, finally \textbf{came}$_{pre}$ off, )}  & When the cast finally \textbf{came}$_{pre}$ off ,  \\
%         & & the patient 's limb would be stiff ... \\
%         error & \multirow{2}{*}{\quad (, to \textbf{get}$_{tgt}$, strength and motion back) }& '' It would take six months of therapy  \\
%         & & to \textbf{get}$_{tgt}$ strength and motion back ... \\
%         & \multirow{2}{*}{(the winter darkness, \textbf{sets}$_{pre}$ in, )} & And as the winter darkness \textbf{sets}$_{pre}$ in ,  \\ 
%         & & and you 're ready to warm up , \\
%         & \multirow{2}{*}{\quad (, \textbf{head}$_{tgt}$, to Ciro \& Sal 's)} & \textbf{head}$_{tgt}$ to Ciro \& Sal 's , where you sit \\
%         & &  near the fireplace and eat the hearty ...  \\ \hline
%         \multirow{8}{*}{Missing} & \multirow{2}{*}{(few, would \textbf{pick}$_{pre}$, Irma Lara)} & ... few would \textbf{pick}$_{pre}$ Irma Lara . \\
%         & & She \textbf{came}$_{tgt}$ to this country illegally \\
%         context & \multirow{2}{*}{\quad (She, \textbf{came}$_{tgt}$, to this country)} & from a small town ... \\
%         & & \\
%         & \multirow{2}{*}{(the tax code, will not \textbf{permit}$_{pre}$, such a loophole)} &	If the tax code will not \textbf{permit}$_{pre}$\\
%         & &  such a loophole , perhaps we could adopt another popular method : \\
%         & \multirow{2}{*}{\quad  (you, would \textbf{earn}$_{tgt}$, rewards points)}& for every hour you spend untangling your budget ,\\
%         & &  or helping others to do so , you would \textbf{earn}$_{tgt}$ rewards points -- redeemable at dozens of national retailers .\\\hline
%         \multirow{2}{*}{Missing} & (I, would \textbf{stop}$_{tgt}$, running)  & My husband asked me whether I would \textbf{stop}$_{tgt}$ running \\
%         & \quad (the doctor, \textbf{told}$_{pre}$, me to) & if the doctor \textbf{told}$_{pre}$ me to . \\
%         discourse cue & (the guy, would \textbf{face}$_{tgt}$, a few problems)  & Viewed though a contemporary lens , the guy born in the church parsonage that now sits across the street  \\
%         & \quad (he, were \textbf{running}$_{pre}$, for president) & from a Dunkin ' Donuts on Bloomfield Avenue would \textbf{face}$_{tgt}$ a few problems if he were \textbf{running}$_{pre}$ for president . \\ \hline
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:error-analysis}
% \end{table*}

%%%%

\eat{
\begin{table*}[ht!]
    \centering
    \begin{tabular}{l|r|r|r} 
        Model & Precision & Recall & F1 \\ \hline \hline
        BERT-feature-1\% & 54.19 & 58.08 & 56.07 \\
        BERT-feature-10\% & 55.45 & 74.76 & 63.67 \\
        BERT-feature-25\% & 58.03 & 80.06 & 67.47 \\
        BERT-feature-50\% & 62.52 & 77.75 & 69.31 \\
        BERT-feature-75\% & 65.20 & 75.08 & 69.79\\ 
        BERT-feature-100\%& 62.81 & 78.95 & 69.95\\\hline
    \end{tabular}
    \caption{Precondition identification result with different sizes of training data.}
    \label{tab:bert-feature-model}
\end{table*}


\begin{table*}[ht!]
    \centering
    \begin{tabular}{l|r|r|r}    
        Model & Precision & Recall & F1 \\ \hline \hline
        BERT-1\% & 50.97 & 51.91 & 51.44 \\
        BERT-10\% & 59.78 & 71.53 & 65.13 \\
        BERT-25\% & 61.45 & 76.65 & 68.21 \\
        BERT-50\% & 64.63 & 75.59 & 69.68 \\
        BERT-75\% & 63.94 & 78.90 & 70.64\\ 
        BERT-100\%& 64.65 & 81.02 & 71.91\\\hline
    \end{tabular}
    \caption{Precondition identification result with different sizes of training data.}
    \label{tab:bert-model}
\end{table*}

\begin{table*}[ht!]
    \centering
    \begin{tabular}{l|r|r|r}
        Context & Precision & Recall & F1 \\ \hline \hline
        Event Trigger  & 54.06 & 75.68 & 63.07 \\
        Event Tuple     & 64.02 & 76.97 & 69.90 \\
        Event Tuple($\pm 1$)    & 63.84 & 78.95 & 70.59  \\
        Sentence        & 64.65 & 81.92 & 71.91 \\
        Sentence($\pm 1$) & 62.69 & 76.92 & 68.47\\
        Sentence($\pm 2$) & 61.65 & 77.33 & 68.60 \\\hline
    \end{tabular}
    \caption{Precondition identification result with different levels of available context.}
    \label{tab:context}
\end{table*}
}
